On the Synthesis of Reactive Collision-Free Whole-Body Robot Motions: A Complementarity-based Approach

This paper is about generating motion plans for high degree-of-freedom systems that account for collisions along the entire body. A particular class of mathematical programs with complementarity constraints become useful in this regard. Optimization-based planners can tackle confined-space trajectory planning while being cognizant of robot constraints. However, introducing obstacles in this setting transforms the formulation into a non-convex problem (oftentimes with ill-posed bilinear constraints), which is non-trivial in a real-time setting. To this end, we present the FLIQC (Fast LInear Quadratic Complementarity based) motion planner. Our planner employs a novel motion model that captures the entire rigid robot as well as the obstacle geometry and ensures non-penetration between the surfaces due to the imposed constraint. We perform thorough comparative studies with the state-of-the-art, which demonstrate improved performance. Extensive simulation and hardware experiments validate our claim of generating continuous and reactive motion plans at 1 kHz for modern collaborative robots with constant minimal parameters.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> related_work.tex <==
\section{Related Literature} \label{sec:rel_work}
Optimization-based motion generation has been thoroughly studied in the literature~\cite{bertsekas2014constrained,lynch2017modern}. One of the pioneering works in this context is the artificial potential fields~\cite{khatib1986real}, and its extensions~\cite{quinlan1993elastic,brock2002elastic}. The current trend in practical scenarios is to utilize robust local optimization techniques~\cite{ratliff2015understanding}. This theme was inspected with a continuous global optimization module in CHOMP (gradient-based)~\cite{ratliff2009chomp} and STOMP (gradient-free)~\cite{kalakrishnan2011stomp}. The authors in TrajOpt~\cite{schulman2013finding}, a SOTA collocation-based trajectory planner, formalize the problem as a non-linear program and utilize Sequential Quadratic Programming (SQP) to come up with a solution. Nevertheless, the design leads to a quadratic increase in computation time as the number of waypoints increases. Furthermore, most methods remain non-realtime and do not encapsulate reactive properties~\cite{sundaralingam2023curobo}. Differently, collision avoidance with Control Barrier Functions has been proposed in~\cite{murtaza2022safety,landi2019safety}. Although suitable for online implementation, their design  often %formulations do not
fails to capture the entire robot and obstacle geometry as we do. Furthermore, as dimensionality increases, CBFs often lead to unfeasible solutions without complex and burdensome parameter tuning. Indeed, it is well-known that small parameter changes can significantly impact system behavior, making it hard to balance safety and performance. Also, in practice, slack variables are often introduced to relax CBF conditions, breaking forward-invariance and further increasing the need for precise tuning, further complicating real-world implementation.   

From a different perspective, 
LCP's have been heavily utilized for robotic applications since its inception in the \textquotesingle$60$s~\cite{lotstedt1982mechanical, moreau1983standard, baraff1994fast}. Standard solvers offering straightforward implementation~\cite{lemke1965bimatrix,murty1988linear} paved the way for formalizing algorithmic rigid body contact models~\cite{lidec2023contact}. However, in the context of motion planning and collision avoidance, they remain largely unexplored. This paper proposes a practical motion planner named FLIQC that exploits a novel kinematic model. FLIQC is able to handle a diverse set of differential constraints and costs. Further, it is scalable to the whole body and is guaranteed to find a local solution if it exists. 
% \begin{figure*}
%     \begin{center}    \includegraphics[width=0.98\linewidth]{figures/drawing_Figure1.pdf}
%     \caption{%
%     Our proposed FLIC planner with real-time collision avoidance. 
% }
%     \label{fig:cover?pic}
%     \end{center}
%     \vspace{-25pt}
% \end{figure*}
Although connecting motion planning with local control is a well-researched problem in the context of mobile robots~\cite{richter2016polynomial}, handling large DoFs is challenging. To this end, the elastic band approach~\cite{brock2002elastic} was strategized to handle obstacles in a mobile manipulation environment. Recently, anytime replanning strategies based on informed sampling strategies have been proposed for continual path improvement in complex scenes~\cite{tonola2023anytime}. Nonetheless, whole-body trajectory optimization with constant minimal parameters in changing environments that captures obstacles and robot shapes is non-existent in the literature.    


